Scaling Synthetic Task Generation for Agents via Exploration

Post-Training Multimodal Large Language Models (MLLMs) to build interactive agents holds promise across domains such as computer-use, web navigation, and robotics. A key challenge in scaling such post-training is lack of high-quality downstream agentic task datasets with tasks that are diverse, feasible, and verifiable. Existing approaches for task generation rely heavily on human annotation or prompting MLLM with limited downstream environment information, which is either costly or poorly scalable as it yield tasks with limited coverage. To remedy this, we present AutoPlay, a scalable pipeline for task generation that explicitly explores interactive environments to discover possible interactions and current state information to synthesize environment-grounded tasks. AutoPlay operates in two stages: (i) an exploration phase, where an MLLM explorer agent systematically uncovers novel environment states and functionalities, and (ii) a task generation phase, where a task generator leverages exploration trajectories and a set of task guideline prompts as context to synthesize diverse, executable, and verifiable tasks. We show AutoPlay generates 20k tasks across 20 Android applications and 10k tasks across 13 applications Ubuntu applications to train mobile-use and computer-use agents. AutoPlay generated tasks enable large-scale task demonstration synthesis without human annotation by employing an MLLM task executor and verifier. This data enables training MLLM-based UI agents that improve success rates up to $20.0\%$ on mobile-use and $10.9\%$ on computer-use scenarios. In addition, AutoPlay generated tasks combined with MLLM verifier-based rewards enable scaling reinforcement learning training of UI agents, leading to an additional $5.7\%$ gain. coverage. These results establish AutoPlay as a scalable approach for post-training capable MLLM agents reducing reliance on human annotation.

==> algorithms/data_pipeline.tex <==

\begin{algorithm}
\caption{Environment-Grounded Task Generation}
\begin{algorithmic}[1] % [1] means line numbers
    \State \textbf{Given:} An Executor Agent \executor, Task Proposer \proposer, Verifier model \verifier, Environment Transition Function $\mathbb{P}$, Taxonomy Prompts $(p_1,....,p_m)$ and generic Exploration Goal $g_{\text{explore}}$
    \State \textbf{Output:} Task Dataset $T = (g_0,..., g_n)$ and a Trajectory Dataset $D = (g_i, \tau_i) \forall i \in n$
    \State \textbf{Initialize:} Task and Trajectory dataset $T = \{\}, D = \{\}$
    \Procedure{execute\_task}{$g$, $\mathbb{P}_e$, $steps$, $env\_context$}
        \State Initialize trajectory $\tau = \{\}$
        \For{$t$ in range$(0, steps)$}
            \State $a_{t} \sim \Cone{\pi_{\text{MLLM}}}(a_t | s_t, g, env\_context)$ 
            \State $s_{t+1} \sim \mathbb{P}_e(s_{t+1} | a_t, s_t)$ 
            \State $\tau = \tau \cup (s_t, a_t)$
        \EndFor
        \State \Return $\tau$
    \EndProcedure
    \For{each environment $e$ in the list}
        \State Explore the environment for $k$ turns for $steps$ steps to gather environment context $\mathcal{T}$
        \For{$i$ in range $(0, k)$}
            \State $\tau_i = \text{Execute\_Task}(g_{\text{explore}}, \mathbb{P}_e, steps, (m_0,...,m_{i-1}))$
            \State $\mathcal{T} = \mathcal{T} \cup \tau_i$
            \State $m_i = f_{\text{memory\_LLM}}(\tau_i)$ \quad // Summarize trajectory to a concise memory representation $m_i$
        \EndFor
        \State Use the environment context to sample a dataset of tasks from task proposer MLLM
        \State $T = T \cup (g_0,...., g_n) \sim \Ctwo{\phi_{\text{MLLM}}}(g_i | \tau_i, p_j) \quad \forall\, i \in k, j \in m$ 

        \State Execute the generated tasks and verify task execution to collect a dataset of trajectories
        \For{$g_i$ in range$(0, T)$}
            \State $\tau_i = \text{Execute\_Task}(g_i, \mathbb{P}_e, steps, ())$  
            \State $(s, cot) = \Cthree{\psi_{\text{MLLM}}}(\tau_i, g_i)$ \quad // Verify if the task execution
            \If{$s = True$}
                \State $D = D \cup \tau_i$ \quad // Add to the trajectory dataset if successful
            \EndIf
        \EndFor
        
    \EndFor
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Environment-Grounded Task Generation}
\begin{algorithmic}[1] % [1] means line numbers
    \State \textbf{Given:} An Executor Agent \executor, Task Proposer \proposer, Environment Transition Function $\mathbb{P}$, Taxonomy Prompts $(p_1,....,p_m)$ and generic Exploration Goal $g_{\text{explore}}$
    \State \textbf{Output:} Task Dataset $T = (g_0,..., g_n)$
    \State \textbf{Initialize:} Task dataset $T = \{\}$
    \For{each environment $e$ in the list}
        \State Explore the environment for $k$ turns for $steps$ steps to gather environment context $\mathcal{T}$
        \For{$i$ in range $(0, k)$}
            \State Initialize trajectory $\tau_i = \{\}$
            \For{$t$ in range$(0, steps)$}
                \State $a_{t} \sim \Cone{\pi_{\text{MLLM}}}(a_t | s_t, g, m_0,...,m_{i-1})$ 
                \State $s_{t+1} \sim \mathbb{P}_e(s_{t+1} | a_t, s_t)$ 
                \State $\tau = \tau \cup (s_t, a_t)$
            \EndFor
            \State $\mathcal{T} = \mathcal{T} \cup \tau_i$
            \State $m_i = f_{\text{memory\_LLM}}(\tau_i)$ \quad // Summarize trajectory to a concise memory representation $m_i$
        \EndFor
        \State Use the environment context to sample a dataset of tasks from task proposer MLLM
        \State $T = T \cup (g_0,...., g_n) \sim \Ctwo{\phi_{\text{MLLM}}}(g_i | \tau_i, p_j) \quad \forall\, i \in k, j \in m$ 
    \EndFor
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Environment-Grounded Synthetic Trajectory Generation}
\begin{algorithmic}[1] % [1] means line numbers
    \State \textbf{Given:} An Executor Agent \executor, Verifier model \verifier, Environment Transition Function $\mathbb{P}$, Task Dataset $T = (g_0,..., g_n)$
    \State \textbf{Output:} Trajectory Dataset $D = (g_i, \tau_i) \forall i \in n$
    % \State Initialize variables
    \State Initialize trajectory dataset $D = \{\}$
    \State Execute the generated tasks and verify task execution to collect a dataset of trajectories
    \For{$g_i$ in $T$}
        % \State $\tau_i = \text{Execute\_Task}(g_i, \mathbb{P}_e, steps, ())$  
        \State Initialize trajectory $\tau_i = \{\}$
        \For{$t$ in range$(0, steps)$}
            \State $a_{t} \sim \Cone{\pi_{\text{MLLM}}}(a_t | s_t, g_i)$ 
            \State $s_{t+1} \sim \mathbb{P}_e(s_{t+1} | a_t, s_t)$ 
            \State $\tau_i = \tau_i \cup (s_t, a_t)$
        \EndFor
        \State $(s, cot) = \Cthree{\psi_{\text{MLLM}}}(\tau_i, g_i)$ \quad // Verify if the task execution
        \If{$s = True$}
            \State $D = D \cup \tau_i$ \quad // Add to the trajectory dataset if successful
        \EndIf
    \EndFor
\end{algorithmic}
\end{algorithm}


==> sections/intro_v0.tex <==
\section{Introduction}

Multimodal Large Language Models (MLLMs) are a promising foundation for building agents across a wide range of downstream domains, including computer use~\citep{qin2025ui,Agent-S,cua2025}, web navigation~\citep{zhou2023webarena,yao2024tau,NEURIPS2022_82ad13ec}, video games~\citep{fan2022minedojo,wang2023voyager}, and robotics~\citep{driess2023palm,black2024pi_0,kim2024openvla}. Owing to their broad knowledge and reasoning capabilities, these models are well-suited to understanding and planning the execution of open-ended tasks across these diverse application areas.

A central challenge in training such agents is the scarcity of downstream interactive agentic data. Such interactive data consists of 
two components: (1.) Diverse Tasks: a sufficiently broad set of tasks or queries that cover real-world use cases of such agents, (2.) Task demonstrations: corresponding task execution trajectory with both efficiency and high fidelity.
For most of these domains, such data is not readily available at web-scale, as much of the relevant interaction data resides on closed systems such as personal devices and commercial hardware. 
%This lack of large-scale, high-quality tasks limits the effectiveness of post-training approaches for agentic MLLMs. 
Consequently, post-training efforts for building agentic MLLMs for such domains have relied heavily on human annotation to source a large pool of diverse tasks and corresponding demonstrations~\citep{li2024effects,wang2025opencuaopenfoundationscomputeruse,qin2025ui}. However, this approach is prohibitively expensive and scales poorly. We argue, the fundamental bottleneck to enable scalable post-training of agentic MLLMs is lack of large pools of high-quality task definition datasets that are diverse, feasible to execute, verifiable, and aligned with real-world use cases. With access to such task datasets, MLLMs could be post-trained in a scalable manner -- either through synthetically generated demonstrations for supervised finetuning (SFT) or via Reinforcement Learning (RL) without any human annotation. This highlights the need for an automatic and reliable pipeline to synthesize tasks at scale.


% Data collection for such domains has two major challenges. The first is defining a sufficiently broad set of tasks or queries for which execution trajectories should be collected; the second is gathering the corresponding trajectories with both efficiency and high fidelity. While task definitions can be partially sourced from humans~\citep{li2024effects,wang2025opencuaopenfoundationscomputeruse}, this approach is prohibitively expensive and scales poorly. An alternate approach is to generate trajectories synthetically~\citep{Trabucco2025InSTA, PAE, pahuja-etal-2025-explorer, xu2024agenttrek, xie2025agentsynth}, but existing approaches suffer from limited diversity, and coverage of the environment. We argue, the fundamental bottleneck for effectively post-training agentic MLLMs is lack of high-quality task definition datasets that are diverse, feasible to execute, verifiable, and aligned with real-world use cases. With access to such datasets, MLLMs could be post-trained more effectively—either through synthetically generated demonstrations for supervised finetuning (SFT) or via Reinforcement Learning (RL). This highlights the need for an automatic and reliable pipeline to synthesize tasks at scale.

%To address this bottleneck, there is a need for an automatic and reliable pipeline to synthesize tasks at scale. 
For such synthesized task datasets to be useful, they must provide broad \emph{coverage} of the target environment, ensuring a diverse and representative training set. They must also be \emph{feasible}, meaning that agents can realistically execute them to generate useful demonstrations. Finally, they should be \emph{verifiable} to filter high-quality trajectories for supervised finetuning or to build a reward model for reinforcement learning. However, building an automatic pipeline that generates tasks with these properties is challenging as it requires explicit knowledge of current state information and  what interactions are feasible in an interactive environment -- knowledge that can only be obtained through direct interaction with the environment. 


%For synthesized tasks to be useful, they must provide broad \emph{coverage} of targeted agentic environment thereby providing the tasks for a diverse and representative training set. The generated tasks must also be \emph{feasible}, meaning that an agent can realistically execute them to produce the desired training data. Finally, tasks should be \emph{verifiable}, such that an appropriate and reliable training signal can be defined.

% In an attempt to address this challenge, prior works have approached this task generation problem by querying an MLLM to generate tasks based on its domain knowledge~\citep{Trabucco2025InSTA,PAE}, this typically yields generic tasks with limited coverage and offers no guarantees of feasibility or verifiability as current MLLMs lack explicit grounding in both environment dynamics and current state information. To address these shortcomings, we propose generating tasks through active exploration of the agent's environment. In this work, we focus on UI agents~\citep{rawles2024androidworld,xie2025agentsynth} that observe the current screenshot and interact with UI elements as a human user would. This setting is both broad, capturing the full spectrum of everyday device tasks and practice since there are programmatic environments available for UI interactions~\cite{rawles2024androidworld,OSWorld}.
In an attempt to address this challenge, prior works have approached this task generation problem by querying an MLLM to generate tasks based on its domain knowledge~\citep{Trabucco2025InSTA,PAE}, this typically yields generic tasks with limited coverage and offers no guarantees of feasibility or verifiability as current MLLMs lack explicit grounding in both environment dynamics and current state information. To address these shortcomings, we propose an approach that actively explores the agent's environment in an exhaustive manner, collecting relevant information that can be used to ground MLLMs in the environment for scalable task generation. In this work, we focus on UI agents~\citep{rawles2024androidworld,xie2025agentsynth} that observe the current screenshot and interact with UI elements as a human user would. This setting is both broad, capturing the full spectrum of everyday device tasks and practice since there are programmatic environments available for UI interactions~\cite{rawles2024androidworld,OSWorld}.

We introduce \autoplay an approach for scalable task generation with a focus on task coverage, feasibility, and verifiability. Our method, depicted in \Cref{fig:teaser}, incorporates two phases of exploration and task generation. 
In the first phase, \emph{environment exploration}, a MLLM explorer agent equipped with memory is prompted to exhaustively explore an increasing number of novel environment states (top of \cref{fig:teaser}). Such exploratory trajectories are intended to discover the functionalities accessible and existing content of the environment. Next, in the \emph{task generation} phase, a task generator MLLM uses exploration trajectories as context of the environment to produce diverse environment-grounded tasks based on a set of task guideline prompts which describe the desired properties of a task (bottom of \cref{fig:teaser}). For instance, in the case of UI agents, a task guideline prompt for Feature-Use tasks would encourage generation of tasks that require doing diverse CRUD (\ie create, edit, of delete) operations on entities in the environment. For example, in a Calendar application, this would lead to tasks that require creating new events with specific parameters (\eg duration, location, etc), updating existing events (\eg adding a reminder to existing meeting) or deleting existing events (\eg delete a certain meeting on certain date or time). We present an example of the exploration trajectory collected by \autoplay and the corresponding tasks synthesized using task generator grounded in the state of the environment in~\cref{fig:qualitative_example}.


\begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{figures/ui-engine.pdf}
    \vspace{2pt}
    \caption{
      \autoplay generates large-scale, diverse and verifiable tasks for scaling supervision for MLLM agents. In stage 1 (top), \autoplay covers the environment states through a MLLM exploration policy that tracks seen states via a memory module. Next, stage 2 (bottom) uses these exploratory trajectories and task guideline prompts as context for proposing tasks. The guidelines help enforce task diversity and the exploration trajectories uncover environment features and content relevant for proposing tasks.
    }
    \label{fig:teaser}
    \vspace{-20pt}
\end{figure}

We use \autoplay to scale task generation for mobile and computer UI agents. \autoplay generates 20k tasks across 20 apps in an Android platform and 10k tasks across 13 apps in a Ubuntu platform. We then synthesize demonstrations for the \autoplay-generated tasks using an MLLM executor and verify them with an MLLM verifier, without relying on privileged environment information or human annotation.
These demonstrations are then used to finetune an MLLM agent with SFT. 
Additionally, \autoplay generated tasks also enables training the MLLM agent with RL, using the MLLM verifier to define an outcome-based reward~\citep{setlur2025rewarding} for each task. Through these experiments we demonstrate \autoplay enables post-training MLLM agents using both SFT and RL in a scalable manner without relying on any human annotation.

We show that \autoplay pipeline substantially improves MLLM agents through fine-tuning. 
In mobile-use, \autoplay boosts success rate performance by $13\%$–$20\%$ over the base model across all model sizes we apply SFT to. 
For computer use, our method improves base model success rate performance by up to $10.9\%$. Beyond SFT, incorporating the generated tasks with the verifier for RL training yields an additional $5.7\%$ improvement in task success rate. Together, these results demonstrate that \autoplay-generated tasks and trajectories lead to consistent and significant performance gains across model sizes and training paradigms.
We also compare the \autoplay task generation pipeline to two different approaches for synthetically generating tasks from prior works for mobile-use domain~\citep{Trabucco2025InSTA,PAE,pahuja-etal-2025-explorer,xie2025agentsynth} which involve either generating tasks with limited environment information or methods that interleave task proposal with execution. 
\autoplay outperforms these methods by $9.4\%$ and $16.6\%$ on success rates respectively. We find this improvement is a result of \autoplay generating tasks with higher diversity, coverage, and feasibility for task execution than prior methods, ultimately yielding datasets that better support the training of capable UI agents. 


==> sections/intro_v1.tex <==
\section{Introduction}


% Post-training Multimodal Large Language Model (MLLMs) as GUI-use agents for mobile-use~\citep{rawles2024androidworld}, computer-use~\citep{OSWorld,qin2025ui,Agent-S}, web environments~\citep{NEURIPS2022_82ad13ec,yao2024tau,Trabucco2025InSTA} offers a promising pathway towards building general-purpose digital assistants. 
% \asn{What if we said GUI-agent instead of GUI-use agent?}
% Such systems can potentially automate complex, multi-turn day-to-day tasks by mirroring the way humans interact with software, potentially changing the way humans interact with these devices.
% \asn{It's not clear to a general audience what you mean by multi-turn here. Use a different phrase or drop it.}
% Training such GUI-use agents is challenging as there are no large-scale GUI interaction datasets with diverse task instructions (\eg ``Add a Meeting with John on Tuesday at 10:00AM to my calendar'') and corresponding demonstrations (\ie sequence of observation, action pairs that demonstrate how to complete a task) readily available on the internet. A common strategy to bridge the data gap is to source high-quality task instructions and corresponding demonstrations in diverse environments (\eg websites, desktop and mobile applications, etc) from human annotators at scale~\citep{li2024effects,qin2025ui,wang2025opencuaopenfoundationscomputeruse}. 
% However, relying on human annotations is prohibitively time-consuming, costly, and ultimately infeasible at internet scale.
% We argue, the fundamental bottleneck in enabling post-training of MLLMs as GUI-use agents lies in the lack of access to large pools of high-quality tasks that are diverse, feasible to execute, verifiable, and aligned with real-world use cases. With access to such tasks, MLLMs could be post-trained to learn from these tasks by generating  demonstrations synthetically for supervised finetuning (SFT) or through trail and error using reinforcement learning (RL). This underscores the need for an automatic and reliable pipeline to synthesize tasks at scale.
% For synthesized tasks to be useful, they must satisfy three key properties: (1) Diverse: tasks should comprehensively cover the entire spectrum of environment functionality, (2) Feasible: tasks should be grounded in possible interactions and current state of the environment to be executable, (3.) Verifiable: tasks should have unambiguous, well-defined goals for reliable evaluation. 
% \asn{I like these criteria. However, I think ``current state of the environment" is too vague.}
% Automatically generating tasks with these properties is difficult because it requires knowledge of what interactions are possible and what is the current state of the environment -- information that can only be obtained through direct interaction with the environment, as it is not directly available on the web. 
% \asn{Why are you mentioning the web here? You already established that no GUI agent data is available on the web.}

Multimodal Large Language Models (MLLMs) provide a highly promising foundation for building agents across a wide range of downstream domains, including computer use~\citep{rawles2024androidworld,OSWorld,qin2025ui,Agent-S}, web navigation~\citep{zhou2023webarena,yao2024tau,NEURIPS2022_82ad13ec}, open-ended games~\citep{fan2022minedojo,wang2023voyager}, and robotics~\citep{zitkovich2023rt,driess2023palm}. Owing to their broad knowledge and reasoning capabilities, these models are well-suited to understanding and planning the execution of open-ended tasks across these diverse application areas.

A central challenge in developing such agents is the scarcity of downstream interactive agentic data. For most of the above domains, readily available web-scale data does not exist, as much of the relevant interaction data resides on closed systems such as personal devices and commercial hardware. Consequently, post-training efforts for agentic MLLMs have relied heavily on either human annotation or synthetic data generation pipelines.

These data collection pipelines face two major challenges. The first is defining a sufficiently broad set of tasks or queries for which execution trajectories should be collected; the second is gathering the corresponding trajectories with both efficiency and high fidelity. While task definitions can be partially sourced from humans~\citep{li2024effects,wang2025opencuaopenfoundationscomputeruse}, this approach is prohibitively expensive and scales poorly. An alternate approach is to generate trajectories synthetically~\citep{Trabucco2025InSTA, PAE, pahuja-etal-2025-explorer, xu2024agenttrek, xie2025agentsynth}, but existing approaches suffer from limited diversity, and coverage of the environment. High-quality task definition datasets that are diverse, feasible to execute, verifiable, and aligned with real-world use cases still remains the fundamental bottleneck for effectively post-training MLLMs. With access to such datasets, MLLMs could be post-trained more effectively—either through synthetically generated demonstrations for supervised finetuning (SFT) or via Reinforcement Learning (RL). This highlights the need for an automatic and reliable pipeline to synthesize tasks at scale.

% Such systems can potentially automate complex, multi-turn day-to-day tasks by mirroring the way humans interact with software, potentially changing the way humans interact with these devices.
% \asn{It's not clear to a general audience what you mean by multi-turn here. Use a different phrase or drop it.}
% Training such GUI-use agents is challenging as there are no large-scale GUI interaction datasets with diverse task instructions (\eg ``Add a Meeting with John on Tuesday at 10:00AM to my calendar'') and corresponding demonstrations (\ie sequence of observation, action pairs that demonstrate how to complete a task) readily available on the internet. A common strategy to bridge the data gap is to source high-quality task instructions and corresponding demonstrations in diverse environments (\eg websites, desktop and mobile applications, etc) from human annotators at scale~\citep{li2024effects,qin2025ui,wang2025opencuaopenfoundationscomputeruse}. 
% However, relying on human annotations is prohibitively time-consuming, costly, and ultimately infeasible at internet scale.
% We argue, the fundamental bottleneck in enabling post-training of MLLMs as GUI-use agents lies in the lack of access to large pools of high-quality tasks that are diverse, feasible to execute, verifiable, and aligned with real-world use cases. 

% (1) Diverse: tasks should comprehensively cover the entire spectrum of environment functionality, (2) Feasible: tasks should be grounded in possible interactions and current state of the environment to be executable, (3.) Verifiable: tasks should have unambiguous, well-defined goals for reliable evaluation. 
% \asn{I like these criteria. However, I think ``current state of the environment" is too vague.}
% Automatically generating tasks with these properties is difficult because it requires knowledge of what interactions are possible and what is the current state of the environment -- information that can only be obtained through direct interaction with the environment, as it is not directly available on the web. 
% \asn{Why are you mentioning the web here? You already established that no GUI agent data is available on the web.}

For synthesized tasks to be useful, we postulate that they must satisfy three key properties. First, tasks should provide broad \emph{coverage} of the domain of interest, thereby provinding the tasks for a diverse and representative training set. Second, the generated tasks must be \emph{feasible}, meaning that an agent can realistically execute them to produce the desired training data. Finally, tasks should be \emph{verifiable}, such that an appropriate and reliable training signal can be defined.

While it is possible to query a foundation model to generate tasks based on its domain knowledge, this typically yields generic tasks with limited coverage and offers no guarantees of feasibility or verifiability. To address these shortcomings, we propose generating tasks through active exploration of an environment that represents the target domain. In this work, we focus on GUI agents~\citep{rawles2024androidworld,xie2025agentsynth}, defined as agents that perform tasks on devices by interacting with UI elements in the same way a human user would. This setting is both broad—capturing the full spectrum of every day tasks a user might perform on a computer—and practical, since programmatic environments for such interactions are readily available.

We introduce \autoplay (see~\Cref{fig:teaser}), an approach for scalable task generation designed geared towards coverage, feasibility, and verifiability. Our method incorporates two central design decisions. First, tasks are generated during an \emph{environment exploration} phase that enables the model to acquire detailed knowledge of the domain. Exploration is carried out by an MLLM prompted to traverse an increasing number of states while proposing tasks along the way. This strategy expands domain coverage, fosters diversity, and naturally supports greater task complexity. In the context of GUI agents, this corresponds to a UI-grounded MLLM exploring applications through direct interaction.

Second, beyond maximizing state coverage, we provide targeted guidance for producing meaningful tasks. This is achieved by specifying a small set of concise, domain-specific prompts—referred to as \emph{task guidelines}—that shape the task generation process during environment exploration. For instance, in the case of GUI agents, a task guideline might encourage the generation of information-seeking tasks, such as answering questions based on information contained within an application.

% MLLMs pre-trained on large-scale web data have shown to be effective at synthesizing tasks across various domains like math~\cite{}, science~\cite{}, and coding~\cite{}. However, naively probing MLLMs to generate tasks for interactive GUI environments often leads to generation of infeasible and ambiguous tasks as these models do not have prior knowledge about possible interactions and current state of the environment. Without access to the \emph{right contextual information} from the environment it is infeasible for an  MLLM to generate high quality tasks to train GUI-use agents. To address this challenge, we propose to explicitly explore the environment while maximizing coverage over possible interactions and discovering novel state information to build the \emph{right} context required by an MLLM to generate environment-grounded tasks. 
% \asn{You say explicitly explore, but are other methods ``implicitly exploring"? I think it's fair to say that other methods don't do any exploration?}
% We call our synthetic task generation pipeline \autoplay, shown in~\Cref{fig:teaser}. 
% \asn{We need to walk the reader through the figure, but we can do this when you update the teaser figure.}
% \autoplay is a two stage approach: (1) \textbf{Environment Exploration}: First, we employ an exploration MLLM agent to exhaustively explore the GUI environment using a generic exploration objective that tasks the agent to maximize functional coverage of the environment, to build \emph{environment context}. The exploration agent receives screen pixel observations from the environment and utilizes a MLLM as a high-level task planner, in conjunction with a GUI grounding model (that maps text description of action to pixel-level coordinates) to generate low-level actions to interact with the environment. (2) \textbf{Exploration Conditioned Task Generation}: In addition to knowledge about what is possible in the environment, the task proposer also needs to provide good coverage over tasks which target the downstream agent skills we care about. 
% For example, the GUI-agent should be able to answer questions in natural language, therefore, the task generator should synthesize tasks that asks questions that require retrieving information from various applications. 
% \asn{This ability to answer questions feels disconnected from the disconnected from a GUI-\emph{agent} which acts to complete goals.}
% To enable this, we introduce a set of \emph{skill taxonomy} prompts (\eg guidelines to generate tasks that require answering questions) in MLLMs context, that steer generation of tasks to provide coverage over target skills we care about. 
% \asn{They way you describe this, it feels like the skill taxonomy prompts are completely targeting the VQA setting and nothing else.}
% Conditioned on the gathered environment context and skill taxonomy prompts, the task proposer MLLM generates a set of tasks for desired agent skills grounded in environment dynamics, state information and functions accessible in the environment. To make \autoplay generally applicable, both the explorer and task proposer agents leverage MLLMs that operate solely on raw visual observations, without relying on any privileged information from the environment. Unlike prior works~\citep{Trabucco2025InSTA,PAE} that rely on pre-trained MLLM knowledge conditioned only on limited environment information (\eg textual descriptions), or methods that interleave task proposal and execution~\citep{pahuja-etal-2025-explorer,xie2025agentsynth}, \autoplay leverages structured exploration explicitly aimed at gathering environment-specific knowledge. 
% \asn{There should be a bit more content about \autoplay is better than prior works. How do the first works only rely on limited environment information? I'm not sure what you mean by limited and why the information \autoplay gets is better. Interleaved task proposal and execution also sounds like a form of exploration. Overall, there needs to be a clearer description of how these prior works fundamentally don't do exploration.}
% This exploration-first approach produces richer context coupled with skill taxonomy prompting to improve task grounding and enabling scalable, high-quality task synthesis.


\begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{figures/ui-engine.pdf}
    %\vspace{-4pt}
    \caption{\textbf{\autoplay}. }
    \label{fig:teaser}
    \vspace{-20pt}
\end{figure}

We apply \autoplay to both SFT- and RL-based agent training on top of an MLLM. For SFT, we synthesize demonstrations for \autoplay-generated tasks using an MLLM executor and verify them with an MLLM verifier. Both the executor and verifier do not rely on any privileged environment information or human annotation, making them easy to scale to any environment. For RL, we similarly use the MLLM verifier to define an outcome reward for each task~\citep{setlur2025rewarding}. In the GUI domain specifically, the executor agent receives visual observations from the environment and employs an MLLM as a high-level task planner, combined with a grounding model that generates low-level actions to produce demonstrations for the assigned tasks. The verifier agent is instantiated with an MLLM that takes as input the task instruction, visual observations, and the action sequence, and outputs whether the task was successful or not.

We demonstrate the effectiveness of \autoplay in both mobile-use~\citep{rawles2024androidworld} and computer-use~\citep{xie2025agentsynth} settings. For mobile use, we generate approximately ${\sim}20\text{k}$ task instructions and ${\sim}8\text{k}$ successful trajectories across only $20$ mobile applications. For computer use, we generate ${\sim}10\text{k}$ task instructions and ${\sim}3.5\text{k}$ successful trajectories across $13$ desktop applications. These results illustrate the scalability of \autoplay in generating diverse tasks and associated training trajectories.
Furthermore, the collected data can be used to substantially improve MLLMs as agents through fine-tuning. For mobile use, \autoplay boosts performance by $13\%$–$20\%$ across all model sizes. For computer use, our method improves base model performance by up to $10.9\%$. Beyond SFT, incorporating the generated tasks with the verifier for RL training yields an additional $5.7\%$ improvement. Together, these results demonstrate that \autoplay-generated tasks and trajectories lead to consistent and significant performance gains across model sizes and training paradigms.

% First, we show how \autoplay enables training MLLMs as mobile-use agents for Android devices and computer-use agents for Ubuntu devices using SFT by enabling synthetic demonstration generation. Using \autoplay, we were able to synthesize ${\sim}20k$ task instructions and ${\sim}8k$ successful trajectories across $20$ mobile applications used in~\cite{rawles2024androidworld} on Android devices. 
% For computer-use domain, we generate ${\sim}10k$ task instructions and ${\sim}3.5k$ successful trajectories across $13$ desktop applications from~\cite{OSWorld} using Ubuntu virtual machines. We finetune a series of Qwen-2.5 VL Instruct~\cite{bai2025qwen25vltechnicalreport} models at 3B-72B scale using \autoplay generated SFT data and find that these models outperform the corresponding base models by up to $14.9\%$ on success rate on AndroidWorld~\cite{rawles2024androidworld} and by $10.9\%$ on success rate on OSWorld~\citep{OSWorld} benchmarks. On mobile-use benchmark, \autoplay-SFT model (7B and 72B) also outperforms competitive UI-TARS 72B~\citep{qin2025ui} and UI-TARS 1.5 7B~\citep{qin2025ui} models that leverage proprietary large-scale human annotated datasets for SFT followed by multi-turn RL.
% Next, we show effectiveness of \autoplay generated tasks combined with MLLM verifier for scaling RL finetuning of mobile-use agents. Specifically, we finetune the \autoplay-SFT 3B model using $8k$ \autoplay generated tasks using GRPO~\citep{deepseek-math} with outcome rewards~\citep{setlur2025rewarding} generated using a Qwen2.5-VL 32B~\citep{bai2025qwen25vltechnicalreport} as task verifier. We find that RL-finetuned models achieve an absolute improvement of $6.7\%$ on success rate over the \autoplay-SFT models on AndroidWorld benchmark, without relying on environment feedback. These results demonstrate how \autoplay is a scalable pipeline to train GUI-use agents without relying on any human annotations.

To understand the impact of design decisions made in \autoplay, we compare \autoplay against two prior approaches for synthetically generating tasks for mobile-use domain~\citep{Trabucco2025InSTA,PAE,pahuja-etal-2025-explorer,xie2025agentsynth}. Specifically, we compare it against methods that use MLLMs conditioned on limited environment information~\citep{PAE,Trabucco2025InSTA} and methods that iteratively explore environments by interleaving task proposal with execution~\citep{pahuja-etal-2025-explorer,xie2025agentsynth}. We find that \autoplay outperforms both of these methods by a large margin, $9.4\%$ and $16.6\%$ on success rates respectively. We identify that the improvement is a result of \autoplay generating tasks with higher diversity, coverage, and execution success rate than prior methods, ultimately yielding datasets that better support the training of capable GUI-use agents. 
Furthermore, we carefully ablate each design decision of our task proposer and show effectiveness of each component showing the effectiveness of exploration and task guidelines.


==> sections/results_old.tex <==
\section{Experiments}

In this section, we demonstrate that \autoplay enables scaling generation of synthetic tasks, that are not only feasible and diverse but also explicitly grounded in environment state and functionality, for GUI-use environments~\cite{rawles2024androidworld,OSWorld} with no human annotations. The resulting high-quality tasks enable scaling of supervised finetuning (SFT) and reinforcement learning (RL) for post-training MLLMs as capable GUI-use agents. 
We also show the tasks synthesized using \autoplay achieve a higher task execution success rate and enable training more capable downstream agents compared to methods that do not explicitly explore the environment~\cite{PAE} and ones that use iterative exploration~\cite{xie2025agentsynth,Trabucco2025InSTA}. Furthermore, we also evaluate importance of exploration and skill taxonomy for task generation and find that both components are important to build a effective task proposer.


\subsection{Mobile-Use}
\label{mobile_use_results}

First, we present the results of training mobile-use agents for Android devices using \autoplay. To do so, we use $20$ mobile applications from the AndroidWorld~\cite{rawles2024androidworld} benchmark as our training environments. For each application, we run the environment exploration for $3$ turns to build the environment context required by the task proposer. In addition, we define $4$ skill taxonomy prompts which describe guidelines for tasks of different categories: (1.) Feature-use: Tasks that use basic features of an app (\eg create/edit/delete events on calendar app), (2.) Information Retrieval: Tasks that require retrieving the requested information and responding in text at the end (\eg How many meetings do I have after 10:00 AM today?), (3.) Repetition: Tasks that require executing same skill multiple times (\eg Add expenses of each grocery item in expense app), (4.) Skill Composition: Tasks with multiple subtasks which require using multiple skills (\eg Add an expense followed by delete an expense in expense app). For each app, exploration turn and skill taxonomy combination we prompt the task proposer to generate up to $50$ tasks, with each task containing $5$ templates maximum. Using this setup, we are able to generate ${\sim}20k$ tasks across these $20$ mobile applications on android devices. 
By executing these ${\sim}20k$ tasks using the task executor and verifying them using the task verifier described in~\cref{sec:executor}, we were able to collect ${\sim}8k$ successful trajectories to train a mobile-use MLLM agent using SFT. To train MLLM agents using RL, we only use the ${\sim}8k$ tasks which were successfully executed by the task executor to reduce the number of infeasible or too hard to execute tasks in our training dataset.

\textbf{Evaluation Setup}. We use the $116$ tasks from AndroidWorld~\cite{rawles2024androidworld} benchmark as our evaluation split. For all  methods, we run evaluation across $5$ random seeds for all $116$ tasks from AndroidWorld. We do this because we find there's high variance when comparing evaluation results across just $1$ seed on AndroidWorld benchmark. For all of our results, we report success rate averaged over $5$ seeds with standard error and Pass@5 success rate.

%Next, we use the synthesized tasks to collect trajectories of task execution using the task executor agent described in~\secref{task_executor}. Finally, we use the task verifier from~\secref{task_verifier} to judge each task execution trace and only keep the successful trajectories. 
%\asn{The previous section just explained your whole pipeline, you don't need to explain it again here.}

\textbf{Effectiveness of \autoplay for SFT}. We present the results of finetuning Qwen2.5-VL MLLMs for mobile-use using SFT in~\tableref{tab:main_results}. The 7B and 72B (rows 7,8) variants of models trained using only ${\sim}8k$ trajectories synthesized using \autoplay achieves $40.1\%$ and $47.9\%$ average success rate on the AndroidWorld benchmark. Our best model (row 9) outperform strong GUI foundation models like UI-TARS 72B and UI-TARS 1.5 7B~\cite{qin2025ui} trained using large-scale human annotated GUI data by $10.2\%$ and $13.7\%$ on average success rate. In addition, our models also outperform the base Qwen2.5-VL Instruct 7B and 72B models (row 5, 6 \vs row 7, 8) by $20.6\%$ and $12.9\%$ on average success rate. Surprisingly, we also find training a 72B model (row 9) on our synthetic data outperforms the teacher model (row 1) by $4.8\%$ on average success rates and by $12.9\%$ on Pass@5 success rates. We present additional analysis for these results in~\secref{mobile_use_results}.
\asn{There should be much more detailed analysis into the results.}

\textbf{Does scaling model size for SFT under fixed data budget help?} Scaling model size on existing datasets has shown consistent improvement in training capable models in various domains~\cite{}. In this experiment, we ask - does the downstream agent performance improve as we scale the size of base model used for finetuning while keeping the size of synthetically generated dataset constant (\ie ${\sim}8k$ trajectories). To test this, we training models of sizes 3B, 7B, 32B, and 72B using SFT on \autoplay generated dataset and evalute the performance on AndroidWorld. We present these results in~\cref{fig:scale_results} (b.), we find that as we scale model size the downstream performance on AndroidWorld keeps improving consistently. Surprisingly, as we scale the finetuning model size past 32B we find that we outperform our data collection policy by $2.5-4.8\%$ on average success rate. 
\asn{I am confused about how we can outperform the expert with SFT? Even if the student was trained with diverse language templates, why would it do better than the expert?}
\asn{I think this detailed scaling study is one of the less interesting results. Certainly the best results for the 72B model should be shared at the start. But showing that performance improves with better scale is a very expected result, so I think it should go at the end of the experiments section. The results on OSW and other analyses are more interesting.}

\textbf{Effectiveness of \autoplay for RL}. Next, we show how \autoplay enables scaling RL training of mobile-use agents. We use ${\sim}8k$ tasks synthesized using \autoplay as our training dataset for RL experiments. As these tasks are synthetically generated we do not have access to environment reward nor is it possible to hand-design rewards for these tasks at such scale. To address this challenge, for each task rollout, we use the task verifier described in~\cref{sec:executor} to verify whether it was successfully executed or not and use it as our outcome reward model~\cite{setlur2025rewarding}. We use GRPO~\cite{} for RL training with $X$ environments, $X$ rollouts per task. We present results of RL finetuning the \textsc{AutoPlay}-SFT agent in~\cref{tab:main_results} (row 9).
We find the SFT$\rightarrow$RL finetuned model achieves $XX\%$ average success rate on AndroidWorld, achieving state-of-the-art results at 7B scale.
% show the effectiveness of this approach, we finetune the base Qwen2.5-VL Instruct 3B and 7B models (row 9 and 10) using $XX$ tasks across $20$ android applications and present evaluation results on AndroidWorld~\cite{rawles2024androidworld} benchmark in~\tableref{tab:main_results}. We find that the 3B and 7B models finetuned using RL achieve $XX\%$ and $YY\%$ average Pass@1 success rates outperforming other methods by $XX\%$ and $YY\%$.


\begin{table}
    \centering
    \resizebox{0.65\linewidth}{!}{
        \setlength\tabcolsep{1pt}
        \begin{tabular}{@{}ll
            % *{2}{>{\centering\arraybackslash}p{0.75cm}}
            *{1}{>{\centering\arraybackslash}p{2.60cm}}
            *{1}{>{\centering\arraybackslash}p{1.80cm}}
            *{1}{>{\centering\arraybackslash}p{0.01cm}}@{}}
                \toprule
                & \textbf{Method} & \textbf{Success Rate} $(\mathbf{\uparrow})$ & \textbf{Pass@5} $(\mathbf{\uparrow})$  \\
                \\[-10pt]
                \midrule
                \rownumber & GPT4o + UI-TARS & $43.1$ & $55.3$ \\
                \midrule
                \rownumber & Seed-VL 1.5     & $62.1$ & $-$ \\
                \rownumber & UI-TARS 2 230B  & $73.3$ & $-$ \\
                \rownumber & UI-TARS 1.5 7B  & $26.4$ {\scriptsize $\pm2.6$} & $36.2$ \\
                \rownumber & UI-TARS 72B     & $37.7$ {\scriptsize $\pm3.4$} & $53.0$ \\
                \rownumber & Qwen-VL 2.5 7B  & $19.5$ {\scriptsize $\pm2.9$} & $27.7$ \\
                \rownumber & Qwen-VL 2.5 72B & $35.0$ {\scriptsize $\pm1.4$} & $43.5$ \\
                \midrule
                \rownumber & \autoplay-3B SFT (Ours) & $34.2$ {\scriptsize $\pm1.6$} & $-$ \\
                \rownumber & \autoplay-7B SFT (Ours) & $40.1$ {\scriptsize $\pm3.3$} & $58.4$ \\
                \rownumber & \autoplay-72B SFT (Ours) & $47.9$ {\scriptsize $\pm1.6$} & $68.2$ \\
                \midrule
                % \rownumber & \autoplay-3B SFT$\rightarrow$RL (Ours) & - & - \\
                \rownumber & \autoplay-3B SFT$\rightarrow$RL (Ours) & $39.9$ & - \\
                \bottomrule
        \end{tabular}
    }
    \vspace{5pt}
    \caption{\textbf{Mobile-Use Results}. Comparison of mobile-use MLLMs finetuned using SFT and RL data generated using \autoplay on AndroidWorld benchmark.}
    \label{tab:main_results}
    % \vspace{-20pt}
\end{table}


\subsection{Computer-Use}

\begin{figure}[t]
  \centering
    \includegraphics[width=1.0\linewidth]{figures/rl_osw_results.png}
    %\vspace{-4pt}
    \caption{\textbf{Results}. (a.) Evaluating RL trained policies with verifier feedback using \autoplay data on AndroidWorld, (b.)  Scaling model size from 3B to 72B for SFT using \autoplay on AndroidWorld, (c.) Comparison of computer-use MLLMs finetuned using SFT data from \autoplay on OSWorld benchmark}
    \label{fig:scale_results}
\end{figure}


In this section, we present results of training computer-use agents for Ubuntu devices using \autoplay. To do so, we use $12$ applications from the OSWorld benchmark~\cite{rawles2024androidworld,qin2025ui} as our training environments. For each application, we run environment exploration for $5$ turns to build the environment context required by our task proposer. In addition, we define $3$ skill taxonomy prompts which describe guidelines for tasks of different categories: (1.) Application-use: Tasks that require broad range of features supported in an application (\eg when proposing tasks for a code editor the tasks should cover modifying app settings, creating new projects, writing code, etc), (2.) Skill Composition: Tasks with multiple subtasks which require chaining multiple skills (\eg Open an existing project in IDE followed by editing a python script), (3.) Content Editing: Tasks that ask the agent to edit content (text, image, video, files) with content specific application (\eg Use image editing tool to crop an image on the device). For each application, exploration turn, and skill taxonomy combination we prompt the task proposer to generate up to $50$ tasks, with each task containing $5$ templates maximum. Using this configuration, we are able to generate ${\sim}10k$ tasks across these $13$ desktop applications on ubuntu devices. We execute these ${\sim}10k$ tasks using our task executor and verifying them using verifier described in~\cref{sec:executor}, we generate ${\sim}3.5k$ successful trajectories to train computer-use MLLM agent using SFT. 

We present the results of finetuning Qwen2.5-VL 7B and 72B MLLMs for computer-use using \autoplay for SFT and evaluating it on OSWorld benchmark~\cite{OSWorld} in~\tableref{tab:main_results}. We use all $369$ tasks from OSWorld benchmark as our evaluation split. We find the \autoplay SFT 7B and 72B models achieve $12.1\%$ and $15.3\%$ success rate, outperforming the base Qwen2.5-VL 7B and 72B models by $8.0\%$ and $10.9\%$ on success rate. In addition, our 72B model also outperforms a powerful GUI model trained using two-stage training pipeline that uses both grounding data and human annotated GUI navigation data by $5.0\%$ on success rate. However, our method still underperforms compared to state-of-the-art GUI foundation models like UI-TARS~\cite{qin2025ui} which uses large scale high-quality human annotated data for computer-use.

% we generate ${\sim}10k$ tasks across $13$ desktop applications on devices with Ubuntu operating system. Next, we use the synthesized tasks to collect trajectories of task execution using the task executor LLM agent described in~\secref{task_executor}. Finally, we use the task verifier from~\cref{task_verifier} to judge each task execution trace and only keep the successful trajectories. 
% \asn{Same comments as for AW. There is no need to re-explain the pipeline. We also need to give details about how the exploration pipeline collected the data.}
% Through this pipeline we collect ${\sim}3.5k$ synthetic trajectories across these $13$ desktop applications to train a computer-use MLLM agent with SFT. Specifically, we use the Qwen2.5-VL Instruct 7B~\cite{bai2025qwen25vltechnicalreport} MLLM as the base model and finetune it using SFT on our dataset to build a end-to-end computer-use MLLM agent that takes image observations as input and outputs low-level mobile actions. 
% \asn{This is repeating from the AW section.}

% We use all $369$ tasks from OSWorld~\cite{rawles2024androidworld} benchmark as our evaluation split. As shown in~\cref{fig:scale_results} (c.), the Qwen2.5-VL Instruct 7B of model finetuned using only ${\sim}3.5k$ synthetic trajectories using our method achieve $12.1\%$ average Pass@1 success rates over $5$ runs on OSWorld benchmark. \todo{Contextualize the results and convey a clear takeaway}



\subsection{Comparison of Synthetic Task Proposers}

In this section, we compare methods for synthetic task generation explored in prior works~\cite{PAE,xie2025agentsynth,Trabucco2025InSTA,pahuja-etal-2025-explorer}. Specifically, different approaches from these prior works are of two categories: (1.) No Exploration: methods that do not use structured exploration to gather information from the environment and instead use simple text descriptions or limited environment context (\eg screenshot of initial page of an application), (2.) Iterative Exploration: methods that interleave task proposal with execution to synthesize environment grounded tasks that are long-horizon. We start by describing the experimental setup for the comparison followed by the exact instantiation of each method for the mobile-use domain.

\textbf{Experimental Setup}. Using each task proposer, we synthesize $5k$ tasks across $20$ applications on Android devices from AndroidWorld~\cite{rawles2024androidworld} benchmark. Next, we use the task executor and verifier described in~\cref{sec:executor} to generate task execution trajectories and verify whether they were successful or not. For each method we only use successful trajectories to build a SFT dataset for training mobile-use MLLM agent by finetuning Qwen2.5-VL 7B using SFT. For models trained using SFT dataset from each method, we run evaluation across $5$ random seeds for all $116$ tasks from AndroidWorld benchmark and report the results in~\cref{tab:proposer_ablate}.

\textbf{No Exploration}. Since MLLMs are trained on large-scale multimodal datasets a common approach for synthetic data generation in various domains is to leverage a MLLM to directly sample datapoints for training. Motivated by this, prior works~\cite{PAE} leverage the internet-scale knowledge of MLLMs to directly sample tasks for interactive environments~\cite{zhou2023webarena,yao2024tau} conditioned on text descriptions of the environment that describes accessible features and possible interactions in the environment. For such methods, the quality of tasks generated depend highly on the environment descriptions provided as context, therefore, these environment descriptions are written by a human annotator to ensure high quality. In order to instantiate this method, we manually write detailed descriptions which includes list of features accessible in each app, we do this for the $20$ android applications we use for training data generation. We provide these app descriptions in addition to a task guidelines (similar to our skill taxonomy) to an LLM and ask it to generate tasks to execute in these apps. We provide the prompt, sample app descriptions, and guidelines in ~\cref{prompts}. Out of the $5k$ synthesized tasks, we find that only $21.3\%$ tasks lead to trajectories that are successful and can be used for SFT.

\textbf{Iterative Explorer}. Methods that do not actively gather information from the environment struggle to propose tasks grounded in environment functionality. To mitigate this challenge, recent works~\cite{pahuja-etal-2025-explorer,xie2025agentsynth} propose a iterative task and trajectory generation pipeline that interleaves task proposal and execution in order to generate tasks that are grounded in what is feasible in the environment and enable execution for complex long horizon tasks. Specifically, these methods start on home page of the application and proposer a short-horizon task based on initial observation, next the task executor agent executes the proposed task. Once the executor completes the proposed subtask the proposer takes over and proposes another short-horizon task using last $3$ observations as input. For each task, we repeat this process upto $k$ times. Finally, a summarizer MLLM takes as input the text description of sequence of subtasks that were executed and whether each of them succeeded or not and proposes a long-horizon goal for the complete trajectory akin to hindsight relabeling. By limiting the task proposer to generate short-horizon tasks and stitching subtasks execution over multiple turns enables data generation for complex long-horizon mobile-use tasks. 

\textbf{\autoplay}. For our method, we use the setup described in~\cref{task_proposer}. Specifically, we run stage 1 of our task proposer for $3$ rounds to explore the app with $4$ skill taxonomy prompts and use each (turn, taxonomy) tuple as context to propose $5k$ tasks. We find that $46.0\%$ of the \autoplay generated tasks lead to trajectories that are successful that can be used for training. \autoplay achieves $25.7\%$ improvement in task execution success rate compared to the No Exploration baseline demonstrates that our task proposer generates larger number of tasks that are feasible to execute in the environment.

\cref{tab:proposer_ablate} shows comparison of using the three task proposers to collect data under fixed budget and train mobile-use agent and its downstream performance on AndroidWorld. Our method (row 3) outperforms both No Exploration and Iterative Explorer  methods by a large margin, $9.4\%$ and $16.6\%$ on average success rate. We attribute this improvement to the ability of \autoplay to propose environment-grounded tasks provide broad coverage over app functionality by active exploration of the environment and skill taxonomy. 
%\autoplay leads to higher task feasibility rate compared to No Exploration task proposer demonstrated by $25.3\%$ higher task execution success rate. This highlights the importance of environment context for generating feasible tasks. 
In contrast, the Iterative Explorer method achieves the lowest success rate. We hypothesize this is due to the difference in distribution of task complexity and length of synthesized trajectories by this method compared to the AndroidWorld benchmark. To investigate this we plot a histogram of trajectory length of dataset generated by Iterative Explorer \vs number of steps required for tasks in AndroidWorld benchmark in~\cref{fig:task_distribution}.

\begin{table}
    \centering
    \setlength\tabcolsep{1pt}
    \begin{tabular}{@{}ll
        *{1}{>{\centering\arraybackslash}p{2.75cm}}
        *{1}{>{\centering\arraybackslash}p{0.01cm}}
        *{1}{>{\centering\arraybackslash}p{2.45cm}}
        *{1}{>{\centering\arraybackslash}p{1.75cm}}
        *{1}{>{\centering\arraybackslash}p{0.01cm}}@{}}
            \toprule
            & & \multicolumn{1}{c}{\textsc{Task Execution}} & & \multicolumn{2}{c}{\textsc{Android World}}  \\
            \cmidrule{3-3} \cmidrule{5-6} 
            & \textbf{Task Generator} & \textbf{Success Rate} $(\uparrow)$ & & \textbf{Success Rate} $(\uparrow)$ & \textbf{Pass@5} $(\uparrow)$  \\
            
            \\[-10pt]
            \midrule
            \rownumber & No Exploration  & $21.3$ &  & $28.8$ {\scriptsize $\pm1.5$} & $49.2$ \\
            \rownumber & Iterative Explorer & -  & & $21.6$ {\scriptsize $\pm1.7$} & $33.6$ \\
            \rownumber & \autoplay & $46.0$ & & $38.2$ {\scriptsize $\pm3.1$} & $58.5$ \\
            \bottomrule
    \end{tabular}
    \vspace{4pt}
    \caption{\textbf{Task Proposer Comparison}. Evaluation results on AndroidWorld comparing MLLM agents trained for mobile-use by finetuning Qwen2.5-VL 7B using SFT data generated by $3$ tasks proposer.}
    \vspace{-10pt}
    \label{tab:proposer_ablate}
\end{table}

\begin{figure}[t]
  \centering
    \includegraphics[width=0.95\linewidth]{figures/analysis.png}
    %\vspace{-4pt}
    \caption{\textbf{Task Diversity Analysis}. 
    }
    \label{fig:task_diversity}
\end{figure}

\subsection{Task Distribution Analysis}

In this section, we analyze the distribution of tasks generated by \autoplay and compare it with task distribution from downstream evaluation benchmarks AndroidWorld and OSWorld and No Exploration task proposer to understand \emph{why} our method is effective and \emph{what} are the areas of improvement. To do so, we annotate each task instruction to list of task categories that describe the task type or skill required to be effective at solving the task using an LLM, in this case GPT-4o~\cite{openai2024gpt4technicalreport}. For example, tasks categorized with type `Composition' require composing multiple skills/subtask to accomplish the overall task (\eg Find when John is free and schedule a meeting with him for this week). We describe each task category with its description in~\cref{supp:task_categorization}. First, we present the comparison of task distribution of \autoplay generated task \vs AndroidWorld and OSWorld benchmark tasks in~\cref{fig:task_diversity} (a) and (b). We plot the percentage of tasks for each task category for both datasets and in addition to percentage of tasks successfully executed by the task executor for \autoplay \vs percentage of tasks successfully executed by the SFT trained \autoplay policy on AndroidWorld and OSWorld respectively. As shown in~\cref{fig:task_diversity} (a), \autoplay provides good coverage over distribution of task categories evaluated by AndroidWorld benchmark. In addition, the task executor performs quite well on majority of task categories except tasks where skills like fine-grained text editing, complex UI interactions (\eg date-time picker wheels, etc), and cross app navigation is required which leads to the downstream policy perform poorly on these task categories. This clearly suggests, improving the task executor while keeping the task generator the same would lead to better quality synthetic dataset to improve downstream agent performance.

In contrast, on OSWorld that is not exactly the case. We find that \autoplay provides decent coverage for common task categories (\eg content or document editing, create, edit, etc) , however, it is not able to generate tasks that provide good coverage over complex categories of tasks that require multi-hop reasoning, cross-app interaction, bash scripting, web search, etc. This suggests there is clearly room for improvement in complex task synthesis. We attribute this gap in task coverage to lack of sufficiently diverse skill taxonomy prompts for computer-use domain. Eventhough the task proposer has access to context from the environment generating such complex tasks requires explicit guidelines to steer the task proposer to generate such tasks by reducing sampling space.

Next, in~\cref{fig:task_diversity} (c) we compare distribution of tasks generated by \autoplay with and without environment exploration. We clearly see a drop in task execution success rates, particularly for task categories such as deleting, editing, or retrieving in-app data, when tasks are synthesized without exploration context, underscoring the importance of grounding tasks in state information from the environment.


\subsection{Importance of task taxonomy}

In addition to using explicit exploration to build environment context, another key component of \autoplay addition is a set of skill taxonomy prompts $(p_1,...,p_m)$ that steer task proposer MLLM to generate tasks of diverse categories and provide coverage over desired skills of downstream agent. To validate impact of this design decision we ablate using \autoplay with and without the skill taxonomy prompt for task dataset generation. Specifically, we run stage 1 of our task proposer for $3$ rounds to explore the app and generate $5k$ tasks across $20$ android applications using \autoplay with and without skill taxonomy prompts in stage two. Next, we collect task execution trajectories using the task executor and verify them using task verifier to only keep successful trajectories. When using the skill taxonomy with \autoplay we achieve $46.0\%$ task execution success rate, in contrast, when we do not use the skill taxonomy we achieve $43.4\%$ task execution success rate. Using the generated datasets, we finetune Qwen2.5-VL 7B using SFT and present evaluation results on AndroidWorld benchmark in~\cref{tab:taxonomy_ablate}. We find that using a skill taxonomy with \autoplay indeed helps improve downstream performance on AndroidWorld benchmark by $10.4\%$. We attribute this improvement in performance to increase in task dataset diversity through use of specific skill taxonomies.

\begin{table}
    \centering
    \setlength\tabcolsep{1pt}
    \begin{tabular}{@{}ll
        *{1}{>{\centering\arraybackslash}p{2.55cm}}
        *{1}{>{\centering\arraybackslash}p{1.85cm}}
        }
            \toprule
            & \textbf{Task Generator} & \textbf{Success Rate} $(\uparrow)$ & \textbf{Pass@5} $(\uparrow)$  \\
            \\[-10pt]
            \midrule
            \rownumber & w/ Skill Taxonomy        & $37.1$ {\scriptsize $\pm3.1$} & $57.5$ \\
            \rownumber & w/o Skill Taxonomy       & $26.7$ {\scriptsize $\pm2.7$} & $38.9$ \\
            \bottomrule
    \end{tabular}
    \vspace{5pt}
    \caption{\textbf{Task Taxonomy Ablation}. Evaluation of mobile-use MLLM agents on AndroidWorld benchmark trained using SFT data generated using \autoplay with and without skill taxonomy prompts.}
    \label{tab:taxonomy_ablate}
\end{table}




